Pupil-driven quantitative differential phase contrast imaging

In this research, we reveal the inborn but hitherto ignored properties of quantitative differential phase contrast (qDPC) imaging: the phase transfer function being an edge detection filter. Inspired by this, we highlighted the duality of qDPC between optics and pattern recognition, and propose a simple and effective qDPC reconstruction algorithm, termed Pupil-Driven qDPC (pd-qDPC), to facilitate the phase reconstruction quality for the family of qDPC-based phase reconstruction algorithms. We formed a new cost function in which modified L0-norm was used to represent the pupil-driven edge sparsity, and the qDPC convolution operator is duplicated in the data fidelity term to achieve automatic background removal. Further, we developed the iterative reweighted soft-threshold algorithms based on split Bregman method to solve this modified L0-norm problem. We tested pd-qDPC on both simulated and experimental data and compare against state-of-the-art (SOTA) methods including L2-norm, total variation regularization (TV-qDPC), isotropic-qDPC, and Retinex qDPC algorithms. Results show that our proposed model is superior in terms of phase reconstruction quality and implementation efficiency, in which it significantly increases the experimental robustness while maintaining the data fidelity. In general, the pd-qDPC enables the high-quality qDPC reconstruction without any modification of the optical system. It simplifies the system complexity and benefits the qDPC community and beyond including but not limited to cell segmentation and PTF learning based on the edge filtering property.

==> sections/sec3_qDCPptf.tex <==
\section{Phase transfer function as edge filters}\label{section 3}
pd-qDPC is based on a proposition of the psf of qDPC experiment: the psf, generated by the Fourier transform of PTF, is a band-limited edge detection filter (twice the size of $NA/\lambda$, NA is the numerical aperture of the image system, $\lambda$ is the wavelength). 

Why this is hold for qDPC? Intuitively, the phase difference of two oblique illuminated images happens on the area where the phase pattern changes rapidly. The differential operation of two phase contrast image in an ideal condition should completely cancel out the background components since they are precisely matched pixel-wisely. Edge structure of the phase pattern can therefore be observed. Similar phenomenon can be also observed in the differential operation of transport of intensity \cite{beleggia2004transport}.

To mathematically illustrate this observation, we consider the property of point spread function $\mathbf{H}_n$ of the differential phase contrast image $\mathbf{S}_n$ in Fourier domain, which is given by 
\begin{equation}
   \mathbf{H}_n(\mathbf{r})=\mathbf{F}^{-1}\widetilde{\mathbf{H}}_n(\mathbf{f}), \label{(4)}
\end{equation}
where $\mathbf{r}=(x,y)$ is the spatial coordinates. $\mathbf{F}^{-1}$ is the inverse Fourier transform. $\mathbf{f}=\left(f_x,f_y\right)$ is the coordinate vector in Fourier space. $\widetilde{\mathbf{H}}_n$ is the  phase transform function (PTF). For qDPC in ideal condition, $\widetilde{\mathbf{H}}_n$ is determined by \cite{tian2015quantitative}:
\begin{equation}
   \widetilde{H}_n(\mathbf{f})=iA\iint q_n(\bm{\uprho})P^*(\mathbf{\bm{\uprho}})
\left [ P(\bm{\uprho}+\mathbf{f}) - P(\bm{\uprho}-\mathbf{f})\right ] \text{d}^2\bm{\uprho}, \label{(5)}
\end{equation}
where A is an energy normalization coefficient. $\otimes$ denotes the 2D convolution. $P$ is the pupil function of the objective lens which is given by
\begin{equation}
P(\mathbf{f})=\text{circ}\left(\frac{\lambda}{NA}\left | \mathbf{f} \right | \right)=
\begin{cases}
 1 & \text{ if } \left | \mathbf{f} \right |<NA/\lambda \\
 0 & \text{ if } \left | \mathbf{f} \right |=elsewise
\end{cases}
,\ \left | \mathbf{f} \right |=\sqrt{f_x^2+f_y^2}. \label{(6)}
\end{equation}


$\mathbf{Q}_n(\mathbf{f})$ is the n-th illumination pupil and is a pure-real odd function which can be expressed as a superposition of a series of dual-delta functions in different position and direction [(as shown in Fig. \ref{Fig.2.} (a)]:
\begin{equation}
\mathbf{Q}_n(\mathbf{f} ) =\int_{0}^{\frac{NA}{\lambda}}\int_{\theta_c-\frac{\pi}{2}}^{\theta_c+\frac{\pi}{2}}
w\left ( \boldsymbol{\rho} \right )\left [ \delta\left ( \mathbf{f}- \bm{\uprho}\right ) - \delta\left ( \mathbf{f}+ \bm{\uprho}\right )  \right ] \rho\text{d}\rho \text{d}\theta, \label{(7)}
\end{equation}
$w\left ( \boldsymbol{\rho} \right )$ is the weight of the pulse and $\bm{\uprho}=(\rho cos\theta,\rho sin\theta)$ is the central of the pulse in Fourier space in polar coordinate. It is also corresponding to the illumination direct of two plane waves. $\theta_c$ controls the illumination direction, and for example, when $w\left ( \boldsymbol{\rho} \right ) = 1$ and $\theta_c=0$, Eq. (\ref{(7)}) generates two half-circles one is positive on the right-hand side of y-axis, and the other one is negative on the left hand side of y-axis as shown in Fig. \ref{Fig.2.} (b).

\begin{figure}
    \centering
    \includegraphics[width = 0.98\textwidth,trim = 0 20 590 0,clip]{Figures/Figure_23.pdf}
    \caption{Decomposition of illumination pupil function $\mathbf{Q}_n$. (a) In first row, $\mathbf{Q}_n$ is expressed as superposition of dual-pulse function of different distance and direction. The yellow arrow denotes positive pulse, and the green arrow denotes the negative pulse. The second row denotes the convolution between $\mathbf{Q}_n$ and $\mathbf{P}$. The third row denotes the corresponding PSF. (b) and (c) show the edge detection feature of PSF/PTF for different PTF layouts, and images.}
    \label{Fig.2.}
\end{figure}

Submit Eqs. (\ref{(7)}), (\ref{(6)}), and (\ref{(5)}) into Eq. (\ref{(4)}) and put all constant coefficients into $C$, we obtain the integral expression of PDF which is 
\begin{equation}
\mathbf{H}_n(\mathbf{r}) =-C\cdot \text{sign}(\mathbf{r}) \frac{J_1\left ( NA k \left | \mathbf{r} \right |  \right ) }
{\left | \mathbf{r} \right |} \int_{0}^{\frac{NA}{\lambda}}\int_{\theta_c-\frac{\pi}{2} }^{\theta_c+\frac{\pi}{2} } 
w\left ( \bm{\uprho} \right ) \sin\left ( 2\pi \bm{\uprho} \cdot \mathbf{r} \right ) \rho \text{d}\rho\text{d}\theta, \label{(8)}
\end{equation}
where $\mathbf{r}=\sqrt{x^2+y^2}$, and $J_1$ denotes the Bessel function of first kind. $k=2\pi / \lambda$. Eq. (\ref{(8)}) implies that the PSF is structured as a superposition of sine-only patterns of differential spatial frequency with no delay, modified by an envelop function $J_1(NA k \left | \mathbf{r} \right |)/\left | \mathbf{r} \right |$.

With Eq.(\ref{(5)}) to Eq. (\ref{(8)}), we have the following 

\begin{lemma} \label{Lemma1}
When $\theta_0 = 0$ the PSF described by Eq. (\ref{(8)}) is an edge detection filter for edge drawing along y-axis, since it produces the highest responce along y-axis when it is filtering with a unit-step function $u(x,y) = \text{sign} (x)$. 
\end{lemma}

\begin{proof}
One has the Fourier spectrum of unit-step function:
\begin{equation}
\widetilde{u} (f_x,f_y)=\begin{cases}
\frac{1}{i f_x}   & f_y = 0\\
 0 & elsewise
\end{cases}. \nonumber
\end{equation}
Combined with (\ref{(5)}) to Eq. (\ref{(7)}) and perform inverse Fourier transform yielding the expression of filter responce $\left|g(x,y)\right|$
\begin{equation}
    \left|g(x,y)\right| = \left| H_n \otimes u \right| = \left| A\int_{0}^{\frac{NA}{\lambda} } \left|\frac{\left \{ \mathbf{P}(\mathbf{f} )\otimes \mathbf{Q}_n(\mathbf{f} ) \right \} |_{f_y=0}}{f_x} \right|
\cos \left ( 2 \pi f_x x \right ) \text{d} f_x  \right| \nonumber
\end{equation} 
note that $\mathbf{P}(\mathbf{f} )\otimes \mathbf{Q}_n(\mathbf{f})  < 0 $ for $f_x \in [0,NA/\lambda]$. following triangle inequality we have
\begin{equation} 
\left|g(x,y)\right| < A \int_{0}^{\frac{NA}{\lambda} } \left|\frac{\left \{ \mathbf{P}(\mathbf{f} )\otimes \mathbf{Q}_n(\mathbf{f} ) \right \} |_{f_y=0}}{f_x} \right|
\left|\cos \left ( 2 \pi f_x x \right )\right| \text{d} f_x \le \left|g(x \equiv 0,y)\right|\nonumber
\end{equation} 
As such, the filter-responce strength becomes the strongest at $x=0$ (along y-axis).

\end{proof}

With Lemma \ref{Lemma1}, we have the following 

\begin{lemma} \label{Lemma2}
For an arbitray $\theta_0=\theta$, the PSF described by Eq. (\ref{(8)}) is an edge detection filter for edge drawing along vector $\mathbf{v}=(-\sin{\theta_c},\cos{\theta_c})$.
\end{lemma}
\begin{proof}
This situation can be deduced to Lemma \ref{Lemma1} if one rotates the PSF as well as the edge around the origin for $\theta$ angle. Then, following Lemma \ref{Lemma1} this is proved. The psf's edge detection is shown in Fig. \ref{Fig.2.} (b) and (c) for different input images.
\end{proof}

% \begin{figure}
%     \centering
%     \includegraphics[width = 0.85\textwidth,trim = 0 20 0 20,clip]{Figures/Fig.3_new.pdf}
%     \caption{Demonstration of qDPC psf's edge detection. The first column denotes the illumination pupil $\mathbf{Q}_n$, the second column denotes the PTF. The third column denotes the PSF. The fourth column denotes the image to be filtered, and the last column denotes the filtering responce.}
%     \label{Fig.3.}
% \end{figure}

Given the edge-detection feature of qDPC's psf, the PTF itself can be used to regularize the solution of qDPC inverse problem, and boosting the phase reconstruction results. As such, we propose the pupil-driven qDPC (pd-qDPC) reconstruction routine to achieve high experimental robustness quantitative phase recovery. 
